Deep Graph Neural Networks via Posteriori-Sampling-based Node-Adaptive Residual Module

Graph Neural Networks (GNNs), a type of neural network that can learn from graph-structured data through neighborhood information aggregation, have shown superior performance in various downstream tasks. However, as the number of layers increases, node representations become indistinguishable, which is known as over-smoothing. To address this issue, many residual methods have emerged. In this paper, we focus on the over-smoothing issue and related residual methods. Firstly, we revisit over-smoothing from the perspective of overlapping neighborhood subgraphs, and based on this, we explain how residual methods can alleviate over-smoothing by integrating multiple orders neighborhood subgraphs to avoid the indistinguishability of the single high-order neighborhood subgraphs. Additionally, we reveal the drawbacks of previous residual methods, such as the lack of node adaptability and severe loss of high-order neighborhood subgraph information, and propose a \textbf{Posterior-Sampling-based, Node-Adaptive Residual module (PSNR)}. We theoretically demonstrate that PSNR can alleviate the drawbacks of previous residual methods. Furthermore, extensive experiments verify the superiority of the PSNR module in fully observed node classification and missing feature scenarios. Our code is available at https://github.com/jingbo02/PSNR-GNN.

==> method.tex <==
\section{The Proposed Method}
\begin{wrapfigure}{r}{6.5cm}
% \begin{figure}[htbp]
	\centering
	\includegraphics[width=0.5\textwidth,page=1]{Pict/PSNR-Arc2.pdf}
	\caption{The framework of PSNR Module}
	\label{fig:architecture}
 \vspace{-1em}
% \end{figure}
\end{wrapfigure}
To solve the above issues, we propose a node-adaptive, model-agnostic, and lightweight residual module named PSNR, which is defined as follows:
% a node-adaptive, general, and lightweight residual module is needed. Based on this concept, we propose a posterior-sampling-based node-level adaptive residual module (PSNR).
\begin{align}
	 \left\{
	  \begin{aligned}
	& \;{\mathbf{H}^{\prime}_{k-1}} = 
	\mathbf{GraphConv}\left(\mathbf{H}_{k-1}\right) \\
	& \;\mathbf{H}_k = \mathbf{H}_{1} + f(diag(\mathbf{\eta}_{k-1}))\left(\mathbf{H}_{1} - \mathbf{H}_{k-1}^{\prime}\right), \;	\mathbf{\eta}_{k-1}
	\sim \mathbf{\mathcal{N}}
	(\mathbf{\mu}_{k-1},{\mathbf{\sigma}_{k-1}}^{2})\\
	& \;\mathbf{\mu}_{k}, \mathbf{\sigma}_{k} = \mathbf{GraphEncoder}_{\mu,  \sigma}(\mathbf{H}_{1} - \mathbf{H}_{k}^{\prime} + \gamma_k \mathbf{LayerEmb}(k)),\\
\end{aligned} \right.
\label{SNR_Defination}
\end{align}
where $\mathbf{H}_k$ is the node representation matrix of the $k$-th layer;
${\mathbf{H}^\prime_k}$ represents the output matrix of any GNN layer with $\mathbf{H}_{k-1}$ as input;
$\eta_k$ represents the node-level residual coefficient at the $k$-th layer, where the element $\eta_k^{(i)}$ corresponds to the residual coefficient at the $i$-th node. In addition, $\eta_k$ follows a high-dimensional Gaussian distribution:
$\mathbf{\mathcal{N}}
(\mu_{k},{\sigma_{k}}^{2})$, and each time before each residual calculation, the distribution is first sampled to obtain the exact residual coefficients.
$\mu_{k}$ and ${\sigma_{k}}$ represent the mean and standard deviation of the distribution, respectively.
$diag(\eta_k)$ represents a diagonal matrix transformed from $\eta_k$, where the $i$-th diagonal element is precisely the $i$-th element of $\eta_k$.
$f(\cdot)$ represents the sigmoid function, which is used to limit the residual coefficient to $(0,1)$.
$\mathbf{GraphEncoder_{\mu, \sigma}}(\cdot)$ is a posterior encoder, which can be any graph convolutional layer (GAT layer~\cite{Velickovic_2017}, GraphSAGE layer~\cite{hamilton2017inductive}, etc.) that is independent of the original GNN model.
$\mathbf{LayerEmb}(k)$ represents the positional encoding with layer number $k$ as input. Its definition is equivalent to \uncite.
$\gamma_k$ is a learnable coefficient serving as the layer encoding factor for the $k$-th layer.

The PSNR module is a concise and plug-and-play universal residual module. As shown in Figure~\ref{fig:architecture}, it is built upon the original backbone model by introducing an encoder after each convolutional operation. This encoder takes the initial convolution result $\mathbf{H}_1$, the intermediate result obtained by the current convolutional layer $\mathbf{H}^\prime_{k-1}$, and the current layer number $k$ as input and outputs the mean $\mu_k$ and variance $\sigma_k$ of the Gaussian distribution to which the current layer's residual coefficient belongs. Subsequently, the residual coefficient can be sampled from this Gaussian distribution, and residual operation can be performed to obtain the output of the current layer. 
% We illustrate the algorithmic process in Figure \ref{fig:architecture}.

The idea behind the PSNR module is to learn a adaptive residual coefficients for each node, thereby achieving finer-grained neighborhood subgraph aggregation to improve the expressive power of GNNs. However, it is noteworthy that directly learning these coefficients for each node through backpropagation is not feasible. 
The main reason is the lack of transferability. Specifically, in settings such as semi-supervised node classification or inductive learning, many or all nodes in the test and validation sets cannot propagate information to the nodes in the training set through multiple message-passing iterations. Therefore, these nodes cannot learn effective coefficients during the training phase. As a remedy, we regard node-level residual coefficients as hidden parameters of the model and attempt to learn the posterior distribution $\mathbf{P}(\eta_k|\mathbf{A}, \mathbf{H}_k, k)$ to which these coefficients belong using an encoder with graph topology and node information as input during the training phase. In most cases, since the training, validation, and test sets originate from the same distribution, the posterior distribution learned about residual coefficients from the training set possesses transferability to the validation and test sets. 
Additionally, it is worth noting that although we consider the posterior distributions of residual coefficients for different layers to be different, we do not parameterize a specific encoder for each layer. Instead, we use the same graph encoder and introduce the layer number $k$ as a positional encoding to differentiate the posterior distributions of residual coefficients for different layers. This design enables our method to circumvent the issue of partial node invisibility during training, as mentioned earlier for node-level learnable residual modules. This gives the PSNR module excellent transferability, enabling it to handle tasks in various scenarios.

To obtain the specific form of PSNR module, We first assume this posterior distribution to be Gaussian:

Considering this, we treat node-level residual coefficients as hidden parameters of the model and attempt to model the posterior distribution $\mathbf{P}(\eta_k|\mathbf{A}, \mathbf{H}_k, k)$ of residual coefficients of different layers using graph topology and node information. We assume this posterior distribution to be Gaussian:
\begin{equation*}
	\mathbf{\eta}_{k}
	\sim \mathcal{N}
	(\mathbf{\mu}(\mathbf{A}, \mathbf{H}_k, k),{\mathbf{\sigma}^{2}(\mathbf{A}, \mathbf{H}_k, k)})
\end{equation*}
Subsequently, to enable back-propagation, we utilize the reparameterization trick, which allows us to express the sampling process from the above distribution as:
\begin{equation*}
	\mathbf{\eta}_{k} = \mathbf{\mu}(\mathbf{A}, \mathbf{H}_k, k) + \zeta \cdot \mathbf{\sigma}(\mathbf{A}, \mathbf{H}_k, k),  \;      
	\zeta \sim \mathcal{N}(0, 1)
\end{equation*}
Furthermore, we parameterize $\mathbf{\mu}(\mathbf{A}, \mathbf{H}_k, k)$ and $\mathbf{\sigma}(\mathbf{A}, \mathbf{H}_k, k)$ as a graph encoder, obtaining the consistent form with Equation \ref{SNR_Defination}. 
%另外值得注意的是，计算出的$k$层的残差系数与$k-1$层的表示经过第$k$层卷积后的结果有关，所以编码器只与一个k-hop邻域子图有关，所以Inductive和图分类认为也可以做，由于缺乏baseline先不放入正文
Furthermore, it is worth noting that although we expect the posterior distributions of residual coefficients for different layers to be different, we did not parameterize a specific encoder for each layer. Instead, we utilized the same graph encoder and introduced the layer number $k$ into the input as a positional encoding to distinguish the posterior distributions of residual coefficients for different layers. This further enhances the expressive power without increasing the model size or memory consumption.


Additionally, our module introduces randomness by sampling residual coefficients during both training and testing phases, thereby adding learnable perturbations to the residual coefficients. This sets it apart from other methods \cite{Rong_2019,DBLP:conf/nips/FengZDHLXYK020,DBLP:conf/aaai/FangX0XY023}, which only incorporate randomness during the training phase and primarily introduce perturbations to node features and graph structure. The specific reasons will be explained later.\uncite

\subsection{Theoretical justifications on
the advantages of the PSNR module}
Next, we will illustrate the advantage of the PSNR module in alleviating over-smoothing. Specifically, we will analyze the expressive power of GCNs using the SNR module, demonstrating that PSNR-GCN achieves the advantage of finely utilizing multiple neighborhood subgraphs aggregation while avoiding the loss of high-order subgraph information.

Firstly, combining with Equation \ref{SNR_Defination}, the matrix form of the recurrence formula for PSNR-GCN can be written as:
\begin{equation*}
	\mathbf{H}_{k}=
	\mathbf{H}_{1} + 
	\Lambda_{k-1}
	\left(
	\mathbf{H}_1 -
	\tilde{\mathbf{D}}^{-1 / 2} \tilde{\mathbf{A}} \tilde{\mathbf{D}}^{-1 / 2}\mathbf{H}_{k-1}
	\right).
\end{equation*}
For simplicity, we use $\Lambda_{k}$ to denote $diag(\eta_k)$.
subsequently, based on this recursive form of formula, we derive the closed-form expression of PSNR-GCN as:
% and demonstrate how SNR-GCN handles multiple neighborhood subgraphs. The closed-form formula for PSNR-GCN can be derived as:
\begin{equation*}
\mathbf{H}_k  = 
\sum_{i=2}^{k-1} \prod_{j=i}^{k-1}\tilde{\mathbf{N}}_j
(
\mathbf{M}_i - 
\mathbf{M}_{i-1}
)
+ \prod_{i=1}^{k-1}\tilde{\mathbf{N}}_i\left( \mathbf{H}_1 + \mathbf{M}_1\right)
-\mathbf{M}_{k-1}, 
\end{equation*} 
where $\tilde{\mathbf{N}}_i = -\Lambda_{k-1} \mathbf{N}$, and 
$
\mathbf{M}_{k} = -\left( 
\Lambda_{k}
\mathbf{N} + \mathbf{I}\right)^{-1}\left(
\mathbf{I} + \Lambda_{k}
\right)\mathbf{H}_{1}
$.
The detailed derivation of this formula can be found in \uncite. 

From the closed-form formula of PSNR-GCN, the first two terms consist of cumulative product terms of different orders, similar to the form of $\mathbf{N}^k\mathbf{H}$, thus approximating a new version of neighborhood subgraph aggregation. Additionally, the formula involves the aggregation of all neighborhood subgraphs from 1 to $k$ hops. This ensures that our method, like other residual methods, can comprehensively utilize the results of multiple neighborhood subgraph aggregations to enhance expressiveness.
Furthermore, since $\Lambda_k$ is a diagonal matrix computed by a learnable posterior encoder with graph structure, node information, and layer number as input, the neighborhood subgraph aggregation of PSNR-GCN is more fine-grained and node-adaptive. This sets it apart from methods like Res, Init-Res, and APPNP.
% , endowing it with stronger expressive power.
Beyond that, we can also demonstrate that the PSNR module can reduce the information loss of high-order subgraph aggregation, thereby further improving the expressive power of GNNs at higher layers.
Specifically, we aim to prove that as the order $k$ increases, the smoothing rate of the cumulative product terms in PSNR is slower than that of the matrix power terms in other methods. Since we are analyzing the smoothing rate, which involves analyzing the asymptotic behavior of cumulative product terms or matrix power terms as the order increases, we can generalize the problem setup. Specifically, we only need to prove the following proposition to support our claim:
\begin{proposition}
Let $\mathcal{S} = \{\mathbf{S}_j = \Lambda_j \mathbf{N} | j \in \mathbb{N}_0 \}$, where $\Lambda_j$ represents a random diagonal matrix with each diagonal element $\Lambda_{j, ii}$ satisfying $0 < \Lambda_{j, ii} < 1$, and let $\mathbf{X}$ be any feature matrix. Then, as the order $k$ increases, the product of elements in the set $\mathcal{S}$ and the matrix $\mathbf{X}$, denoted as $\mathbf{X}^{(k)} = \prod_{i=1}^{k} \mathbf{S}_i \mathbf{X}$, converges to a rank-one matrix with identical rows slower than $\mathbf{X}_{GCN}^{(k)} = \mathbf{N}^k\mathbf{X}$.
\end{proposition}
Since the diagonal elements of the diagonal matrix $\Lambda$ are all results of the sigmoid function, we can assume that they have a lower bound $\epsilon > 0$. Therefore, in this setting, each element $\mathbf{S}_i$ in the set $\mathcal{S}$ is a row-stochastic matrix satisfying the following property:
\begin{property}
    For a row-stochastic matrix $\mathbf{S}_k$, there exists an $\epsilon > 0$ satisfying the following conditions:\\
1. $\epsilon \leq \mathbf{S}_{k,ij} \leq 1$, if $(i,j) \in \mathcal{E}$,\\
2. $\mathbf{S}_{k,ij} = 0$, if $(i,j) \notin \mathcal{E}$,
\end{property}
Due to the existence of \textbf{Property 1}, we can refer to the work of \citeauthor{DBLP:conf/nips/WuAWJ23}. \citeauthor{DBLP:conf/nips/WuAWJ23} describes the attention matrix of GAT as a row-stochastic matrix satisfying Property 1, and leveraging mathematical tools such as joint spectral radius from the perspective of dynamical systems, it proves that the convergence rate of GAT is bounded below by GCN. This conclusion can be used to prove \textbf{Proposition 1}, thereby demonstrating that the PSNR module can alleviate the loss of high-order neighborhood subgraph information.
Furthermore, this conclusion also explains why randomness is introduced during both the training and testing phases. It further reduces the smoothing rate through random perturbations, thereby enhancing the model's expressive power.

% \begin{displaymath}
%     p_{k-1}^{(i)}
%     \sim \mathbf{\mathcal{N}}
%     (\mathbf{\mu}^{(i)}_{k-1},{\mathbf{\sigma}^{(i)}_{k-1}}^{2}),
% \end{displaymath}
% where $\mathbf{h}_k^{(i)}$ denotes the representation of \emph{k}-th layer of node $i$, 
%  ${\mathbf{h}_k^{(i)}}^\prime$ denotes the result obtained by an arbitrary GNNs layer with $\mathbf{h}_{k-1}^{(i)}$ as input. $p_k^{(i)}$ is a random number sampled from $\mathbf{\mathcal{N}}
%     (\alpha^{(i)}_{k},{\beta^{(i)}_{k}}^{2})$, which associated with the $i$-th node at the \emph{k}-th layer, and $\alpha^{(i)}_{k} $ and ${\beta^{(i)}_{k}}$ are learnable parameters representing the mean and the standard deviation of this distribution, respectively. It is noteworthy that our module introduces randomness during both the training and testing phases by sampling residual coefficients, which sets it apart from other methods \cite{Rong_2019,DBLP:conf/nips/FengZDHLXYK020,DBLP:conf/aaai/FangX0XY023} that only incorporate randomness during the training phase. Next, we will illustrate the superiority of the SNR module in terms of flexibility and overfitting alleviation.




% \subsection{Flexibility}
% In this section, an analysis of the expressive power of GCN with the SNR module will be conducted, demonstrating that SNR-GCN achieves a more flexible utilization of multiple neighborhood subgraph aggregations.
% First of all, combined with Eq.~\ref{SNR_Defination}, the matrix form of the recurrence formula of SNR-GCN can be written as:
% \begin{equation}
% \mathbf{H}_{k}=
% \mathbf{H}_{1} + 
% \Lambda_{k-1}
% \left(
% \mathbf{H}_1 -
% \tilde{\mathbf{D}}^{-1 / 2} \tilde{\mathbf{A}} \tilde{\mathbf{D}}^{-1 / 2}\mathbf{H}_{k-1}
% \right),
%  \end{equation}
% where $\Lambda_k $ is a diagonal matrix whose $i$-th diagonal element is equal to $p_k^{(i)}$. We first try to obtain the general formula of SNR-GCN according to the recursive formula and demonstrate SNR-GCN's treatment of multiple neighborhood subgraph aggregations. The general formula of SNR-GCN can be deduced as:
%     $     
%     \mathbf{H}_k  = 
%     \sum_{i=2}^{k-1} \prod_{j=i}^{k-1}\tilde{\mathbf{N}}_j
%     (
%     \mathbf{M}_i - 
%     $
%     $
%     \mathbf{M}_{i-1}
%     )
%     + \prod_{i=1}^{k-1}\tilde{\mathbf{N}}_i\left( \mathbf{H}_1 + \mathbf{M}_1\right)
%     -\mathbf{M}_{k-1}, 
%     $
%     where $\tilde{\mathbf{N}}_i = -\Lambda_{k-1} \mathbf{N}$ and 
%     $
%     \mathbf{M}_{k} = -\left( 
%     \Lambda_{k}
%     \mathbf{N} + \mathbf{I}\right)^{-1}\left(
%     \mathbf{I} + \Lambda_{k}
%     \right)\mathbf{H}_{1}.
%     $
% The details of the derivation are provided in Appendix \hyperref[Appendix D]{D}. From the general formula of SNR-GCN,  it is evident that $\mathbf{M}_{k}$ is a linear transformation of $\mathbf{H}_1$. Therefore, the first two terms of the formula
% can be approximately regarded as a new form of neighborhood subgraph aggregation.  Moreover, it is evident that all 1 to $k$ hop neighborhood subgraph aggregations appear in the formula. This ensures that our approach, like other residual models, can effectively utilize multiple neighborhood subgraph aggregations. 
% Further, because $\Lambda_k$ are learnable diagonal matrixes, SNR-GCN's neighborhood subgraph aggregation is learnable and more 
% flexible, which further makes expressive power stronger. 

% It's worth noting that when $\Lambda_k = -\alpha\mathbf{I}$, the first term becomes 0, and the remaining terms are equivalent to APPNP's formula. This implies that SNR-GCN can be approximated as a finer-grained and more expressive version of APPNP.

% \subsection{Overfitting Alleviation}
% Another key point of SNR is that it introduces randomness to alleviate overfitting.
% In our initial idea, we attempt to construct a generic module resembling the initial residual at the node level. Based on this premise, the following modules were initially designed:
% \begin{equation}
%     \mathbf{h}_k^{(i)} = \mathbf{h}_{1}^{(i)} + \mathbf{sigmoid}(q_k^{(i)})
% \left(\mathbf{h}_{1}^{(i)} - {\mathbf{h}_{k-1}^{(i)}}^{\prime}\right), 
% \end{equation}
% where $q_k^{(i)}$ is a learnable parameter which associated with the $i$-th node at the \emph{k}-th layer. However, as shown in section ~\ref{section5.5}, the model has a high risk of overfitting when adding this module. Additionally, we also observe that
% initially learning a normal distribution associated with the residual coefficient $q^{(i)}_k$ using the reparameterization trick and obtaining specific value through sampling in each computation ranther than directly training $q^{(i)}_k$ through backpropagation, resolves the issue and significantly enhances the model's performance.

% It is worth noting that GCNII and SNR-GCN share a similar architecture, so both can be viewed approximately as more refined APPNP-style models. However, when faced with the problem of overfitting due to more parameters, GCNII adds an identity matrix to mitigate the issue. Later experiment results have shown that SNR-GCN's learning distribution-sampling approach is more effective in alleviating overfitting.


\subsection{Complexity Analysis}
Furthermore, as described in the definition section of \uncite, our method only introduces a single-layer graph posterior encoder to achieve the computation of multi-layer residual coefficients and the learning of multi-order neighborhood subgraph information. Compared to dense methods, our approach requires fewer additional parameters and does not need to store intermediate results, thereby significantly reducing unnecessary memory consumption, improving training efficiency, and enhancing the scalability of the method. Next, we will use PSNR-GCN as an example to provide a complexity analysis of the PSNR module.
% \textbf{Model Complexity.} According to Eq.~\ref{SNR_Defination}, at each layer the PSNR module learns a mean and standard deviation of the corresponding distribution for each node, so the complexity can be calculated as \emph{O}(\emph{n}), and thus the additional complexity of the \emph{k}-layer model equipped with PSNR is \emph{O}(\emph{kn}).
% \textbf{Time Complexity.} 
The time complexity of a vanilla GCN layer mainly comes from the matrix multiplication of \textbf{N} and \textbf{H}, hence its complexity is \emph{O}$(n^2d)$. And the main computational parts of a SNR module are the sampling of $p_k^{(i)}$, scalar multiplication and matrix addition, which correspond to a complexity of \emph{O}(\emph{n}), \emph{O}(\emph{nd}), and \emph{O}(\emph{nd}), respectively. Thus the time complexity of the SNR module is \emph{O}(\emph{nd}) and the time complexity of a GCN layer equipped the SNR module is \emph{O}($n^2d+nd$). We also show the specific running time in Appendix \hyperref[Appendix E]{E}, indicating that the SNR module barely affects the computational efficiency.

% \subsection{Comparing with other subgraph-based methods\tdb}

% It is worth noting that a lot of previous work mentions "subgraph". However, our approach is fundamentally different from these approaches.

% \textbf{Relation with other subgraph-based methods.} While there are existing works \cite{DBLP:conf/iclr/BevilacquaFLSCB22, DBLP:conf/nips/QianRGN022} related to subgraphs, they primarily focus on graph classification tasks, aiming to learn representations of entire graphs. Given the limited capacity of GNNs to effectively represent the entire graphs, these subgraph-based approaches employ various strategies to leverage information from multiple subgraph structures within the overall graph to improve the representation.

% In contrast, our focus is on node-level tasks, specifically, enhancing the representations of individual nodes. In our context, we naturally refer to neighborhood subgraphs as different orders of ego-networks centered on a node (which can be regarded as subgraphs of the entire graph). Our work uncovers the relationship between these subgraphs and oversmoothing, as well as how to utilize them to enhance node representations. This distinction fundamentally sets our approach apart from other subgraph methods.



